DeepOPF: A Deep Neural Network Approach for Security-Constrained DC Optimal Power Flow

We develop DeepOPF as a Deep Neural Network (DNN) approach for solving security-constrained direct current optimal power flow (SC-DCOPF) problems, which are critical for reliable and cost-effective power system operation.DeepOPF is inspired by the observation that solving SC-DCOPF problems for a given power network is equivalent to depicting a high-dimensional mapping from the load inputs to the generation and phase angle outputs. We first train a DNN to learn the mapping and predict the generations from the load inputs. We then directly reconstruct the phase angles from the generations and loads by using the power flow equations. Such a predict-and-reconstruct approach reduces the dimension of the mapping to learn, subsequently cutting down the size of the DNN and the amount of training data needed. We further derive a condition for tuning the size of the DNN according to the desired approximation accuracy of the load-generation mapping. We develop a post-processing procedure based on $\ell_1$-projection to ensure the feasibility of the obtained solution, which can be of independent interest. Simulation results for IEEE test cases show that DeepOPF generates feasible solutions with less than 0.2% optimality loss, while speeding up the computation time by up to two orders of magnitude as compared to a state-of-the-art solver.

==> backup.tex <==
\begin{table*}[!t]
	\centering
	%\tiny
	\caption{{Performance Evaluation and Comparison on The Active Power Increase (API) Cases. This table will be updated soon.}}
	\renewcommand{\arraystretch}{1.4}
	\begin{threeparttable}
		\begin{tabular}{c|c|c|c|cc|c|cc|c}
			\toprule
			\hline
			\multirow{2}{*}{Case} &
			\multirow{2}{*}{\tabincell{c}{\# Contingencies}} &
			\multirow{2}{*}{\tabincell{c}{\# Variables}} &
			\multirow{2}{*}{\tabincell{c}{Feasibility (\%)}} &
			\multicolumn{2}{c|}{\tabincell{c}{Average cost (\$/hr)}} &
			\multirow{2}{*}{\tabincell{c}{Optimality \\loss (\%)}} &
			\multicolumn{2}{c|}{\tabincell{c}{Running time (millisecond)}} &
			\multirow{2}{*}{\tabincell{c}{Speedup}} \\
			\cline{5-6} \cline{8-9}
			&&&&\textsf{DeepOPF}&Ref.&&\textsf{DeepOPF}&Ref.&\\
			\hline
			\tabincell{c}{IEEE Case30} &29& 902& &  & 1275.1 &&  & {21} & $\times  $\\%0.0272
			\hline
			\tabincell{c}{IEEE Case57} &78&4507& & & 49307.8 & &  & {111} & $\times  $\\%0.0665
			\hline
			\tabincell{c}{IEEE Case118}&157&18663&   &   &  &  &   &   & $\times  $ \\ %0.482
			\hline
			\tabincell{c}{IEEE Case300}&235&70857&   &   &   &   &   &   & $\times  $ \\ 
			\hline		
			\bottomrule
		\end{tabular}
		%\begin{tablenotes}
		%\footnotesize
		%\item[*] Running time is the average computation time of all test instances.
		%\end{tablenotes}
		\end{threeparttable}
	\label{table3}
\end{table*} 


\begin{table*}[!t]
	\centering
	%\tiny
	\caption{{Performance Evaluation and Comparison on The Neuron Network Size for IEEE 118 Test Case under The Active Power Increase Cases. This table will be updated soon.}}
	\renewcommand{\arraystretch}{1.4}
	\begin{threeparttable}
	\resizebox{\textwidth}{15mm}{
		\begin{tabular}{c|ccc|ccc|ccc|ccc}
			\toprule
			\hline
			\multirow{2}{*}{DNN size} &
			\multicolumn{3}{c|}{\tabincell{c}{\# Neurons}} &
			\multicolumn{3}{c|}{\tabincell{c}{\# Neurons}} &
			\multicolumn{3}{c|}{\tabincell{c}{\# Neurons}} \\
			\cline{2-10}
			&{Feasibility (\%)}&{Optimality loss (\%)}&{Speedup}&{Feasibility (\%)}&{Optimality loss (\%)}&{Speedup}&{Feasibility (\%)}&{Optimality loss(\%)}&{Speedup}\\
			\hline
			\tabincell{c}{\# Layers} &29& 902& &  & 1275.1 &&  & {21} & $\times  $\\%0.0272
			\hline
			\tabincell{c}{\# Layers} &78&4507& & & 49307.8 & &  & {111} & $\times  $\\%0.0665
			\hline
			\tabincell{c}{\# Layers}&157&18663&   &   &  &  &   &   & $\times  $ \\ %0.482
			\hline
			\tabincell{c}{\# Layers}&235&70857&   &   &   &   &   &   & $\times  $ \\ 
			\hline		
			\bottomrule
		\end{tabular}}
		%\begin{tablenotes}
		%\footnotesize
		%\item[*] Running time is the average computation time of all test instances.
		%\end{tablenotes}
		\end{threeparttable}
	\label{table3}
\end{table*} 


\begin{table}[!t]
	\caption{{Analysis of Different Combinations of Weights. This table is used for the corresponding simulations with different combinations of weights.}}
	\renewcommand{\arraystretch}{1.5}
	%\scriptsize
	\centering
		\begin{tabular}{c|c|c|c}
		\hline
		\multirow{3}{*}{Variant}
		& \multicolumn{3}{c}{Active Increase Condition}\\
		\cline{2-4}
		&\tabincell{c}{Feasibility Rate \\(\%)} & \tabincell{c}{Optimality loss \\(\%)} & Speedup\\
		\hline		
		\textsf{}-V1 & & & \\
		\hline
		\textsf{}-V2 & & & \\
		\hline
		\textsf{}-V3 & & & \\
		\hline
	\end{tabular}
	\label{table6}
    \end{table}

% \begin{table*}[!t]
% \caption{\rev{Analysis of Different Combinations of NN size and the amount of training data.}}
% \resizebox{\textwidth}{!}{
% \begin{threeparttable}[b]
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{3}{*}{} & \multicolumn{9}{c|}{Typical Operation Condition}& \multicolumn{9}{c}{Active Increase Condition} \\
% \hline
% & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}l@{}}Prediction \\ error\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}l@{}}Running \\
% time\end{tabular}} & \multicolumn{3}{c|}{Speedup} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}l@{}}Prediction \\
% error\end{tabular}} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}l@{}}Running \\ time\end{tabular}} & \multicolumn{3}{c}{Speedup} \\
% \hline
% & V1& V2& V3& V1& V2& V3& V1& V2& V3& V1& V2& V3& V1& V2& V3& V1& V2& V3\\
% \hline
% && && &&&&&&& &&&&&&& \\       
% \hline
% \end{tabular}
% \end{threeparttable}}
% \end{table*}
